Representation Sparsification with Hybrid Thresholding for Fast SPLADE-based Document Retrieval

Learned sparse document representations using a transformer-based neural model has been found to be attractive in both relevance effectiveness and time efficiency. This paper describes a representation sparsification scheme based on hard and soft thresholding with an inverted index approximation for faster SPLADE-based document retrieval. It provides analytical and experimental results on the impact of this learnable hybrid thresholding scheme.

==> table/baseline.tex <==
\begin{table}[tpbh]
\footnotesize
    \centering
        \caption{Baseline Methods.}
\label{tab:baseline}
% \resizebox{1.05\columnwidth}{!}{%
    \begin{tabular}{l|c|c|c|cc}
    \hline
     & \textbf{MRR@10} & \textbf{MRT, $k=10$} & \textbf{MRT, $k=1000$} & ql & dl \\ 
     \hline 
    ECAI20 Paper &  \\
    Top-k-post &  \\
        -305 & 0.3962 & 42.4(202) & 114(369) & 13.7(89) & 277\\
        -200 & 0.3960 & 37.2(166) & 94.9(314) & 13.7(89) & 197 \\
        -150 & 0.3933 & 28.6(138) & 80.6(260) & 13.7(89) & 149 \\
        -100 & 0.3908 & 21.8(106) & 62.5(196) & 13.7(89)  & 99 \\
    Top-k-joint &  \\

     \hline
    \end{tabular}
    % }
\end{table}

==> table/lambda_t.tex <==
\begin{table}[tpbh]
\footnotesize
    \centering
        \caption{$\lambda_t$.}
\label{tab:lambdat}
% \resizebox{1.05\columnwidth}{!}{%
    \begin{tabular}{l|c|c|c}
    \hline
     & \textbf{MRR@10} & \textbf{MRT, $k=10$} & \textbf{MRT, $k=1000$}  \\ 
     \hline 
    1 & 0.3955 \\
    2 &  \\
    3 & 0.3942 & \\
    5 &  & \\
    10 &  & \\
     \hline
    \end{tabular}
    % }
\end{table}

==> table/temp.tex <==
\begin{table}[tpbh]
\footnotesize
    \centering
        \caption{Temprature.}
\label{tab:softvshard}
% \resizebox{1.05\columnwidth}{!}{%
    \begin{tabular}{l|ccc|cc}
    \hline
     & \textbf{MRR@10} & \textbf{MRT, $k=10$} & \textbf{MRT, $k=1000$} & \textbf{ql} & \textbf{dl} \\ 
     \hline 
    K=2.5-$H$ & 0.3947 & & & 11.5 & 149 \\
    K=2.5-$\widehat{H}$ & 0.3963 & & & 11.5 & 421  \\
    K=25-$H$ & 0.3955 & 22.8(108) & 62.3(195) & 11.3(48) & 140 \\
    K=25-$\widehat{H}$ & 0.3961 & 28.7(136) & 76.9(239) & 11.3(48) &  \\
    K=250-$H$ & 0.3946 & & &  11.2 & 135 \\
    K=250-$\widehat{H}$ & 0.3947 & & & 11.2 & 139 \\

     
     \hline
    \end{tabular}
    % }
\end{table}
